Observation of electroweak $W^{\pm}Z$ boson pair production in association with two jets in $pp$ collisions at $\sqrt{s} =$ 13 TeV with the ATLAS detector

An observation of electroweak $W^{\pm}Z$ production in association with two jets in proton-proton collisions is presented. The data collected by the ATLAS detector at the Large Hadron Collider in 2015 and 2016 at a centre-of-mass energy of $\sqrt{s} =$ 13 TeV are used, corresponding to an integrated luminosity of 36.1 fb$^{-1}$. Events containing three identified leptons, either electrons or muons, and two jets are selected. The electroweak production of $W^{\pm}Z$ bosons in association with two jets is measured with an observed significance of 5.3 standard deviations. A fiducial cross-section for electroweak production including interference effects is measured to be $\sigma_{WZjj\mathrm{-EW}} = 0.57 \; ^{+ 0.14} _{- 0.13} \,(\mathrm{stat.}) \; ^{+ 0.07} _{- 0.06} \,(\mathrm{syst.}) \; \mathrm{fb}$. Total and differential fiducial cross-sections of the sum of $W^\pm Z jj$ electroweak and strong productions for several kinematic observables are also measured.

==> journal/Makefile <==
# Makefile for creating an ATLAS paper draft using journal classes

TEXLIVE  = 2016
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = bibtex
DVIPS    = dvips
DVIPDF   = dvipdf
OPEN     = open

TEXFILES = $(wildcard *.tex)

.PHONY: texlive clean

all: atlas-elsevier atlas-jhep atlas-revtex

texlive:
	for file in $(TEXFILES); do \
	  if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	    echo "Changing texlive value in $$file"; \
	    sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $$file; \
	  else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \
	done

atlas-elsevier: atlas-elsevier.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-jhep: atlas-jhep.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-revtex: atlas-revtex.pdf
	@echo "Made $<"
	# $(OPEN) $<

run_latex: $(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $< and $(basename $<).pdf"

# Standard LaTeX targets
%.pdf: %.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.dvi: $(BASENAME).tex
	$(LATEX)    $<
	$(LATEX)    $<

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf \
	 *.spl *-revtexNotes.bib *.run.xml *.synctex.gz *~

cleanall: clean
	-rm *.pdf


==> journal/atlas-document-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used by the different cover pages.
%-------------------------------------------------------------------------------

%% Title
\AtlasTitle{A simple ATLAS paper draft}
%
% Author - this does not work with revtex
% \author{The ATLAS Collaboration}
%
% Date: if not given, uses current date
% \date{\today}

% Draft version:
% Should be 1.0 for the first circulation, and 2.0 for the second circulation.
% If given, adds draft version on front page, a 'DRAFT' box on top of each other page, 
% and line numbers.
% Comment or remove in final version.
\AtlasVersion{1.0}

% ATLAS reference code, to help ATLAS members to locate the paper
\AtlasRefCode{GROUP-2014-XX}

% ATLAS note number. Can be an COM, INT, PUB or CONF note
% \AtlasNote{ATLAS-CONF-2014-XXX}
% \AtlasNote{ATLAS-PUB-2014-XXX}
\AtlasNote{ATLAS-COM-PHYS-2014-XXX}

% Submission journal
\AtlasJournal{Phys.\ Lett.\ B.}

% Abstract - % directly after { is important for correct indentation
\AtlasAbstract{%
	This is a bare bones ATLAS document used to demonstrate how to use journal templates.

	This document is typeset using the \DocumentStyle.
}

%-------------------------------------------------------------------------------
% The following information is needed for the cover page. The commands are only defined
% if you use the coverpage option in atlasdoc or use the atlascover package
%-------------------------------------------------------------------------------

% Explicit list of supporting notes  (leave as null \AtlasCoverSupportingNote{} if you want to skip this option)
\AtlasCoverSupportingNote{A supporting note}{http://cds.cern.ch/record/XXXXXX}
\AtlasCoverSupportingNote{Another supporting note}{http://cds.cern.ch/record/YYYYYY}
%
% OR (the 2nd option is deprecated, especially for CONF and PUB notes)
%
% Supporting material TWiki page  (leave as null \AtlasCoverTwikiURL{} if you want to skip this option)
% \AtlasCoverTwikiURL{https://twiki.cern.ch/twiki/bin/view/Atlas/WebHome}

% Comment deadline
\AtlasCoverCommentsDeadline{DD Month 2014}

% Analysis team members - contact editors should no longer be specified
% as there is a generic email list name for the editors
\AtlasCoverAnalysisTeam{Peter Analyser, Susan Editor1, Jenny Editor2, Alphonse Physicien}

% Editorial Board Members - indicate the Chair by a (chair) after his/her name
\AtlasCoverEdBoardMember{EdBoard~Chair~(chair), EB~Member~1, EB~Member~2, EB~Member~3}

% Editors egroup
\AtlasCoverEgroupEditors{atlas-GROUP-2014-XX-editors@cern.ch}

% EdBoard egroup
\AtlasCoverEgroupEdBoard{atlas-GROUP-2014-XX-editorial-board@cern.ch}

% CERN preprintnumber
\PreprintIdNumber{CERN-EP-2014-XX}


==> sections/LLHprofile.tex <==

\begin{figure}[!htbp]
\begin{center}
 \includegraphics[width=.7\textwidth]{figures/AuxFigs/NLL_CombinedFit_FINAL.pdf}
\end{center}
\caption{The profile of the negative log-likelihood ratio $L(\mu_{\wzjjew})$ of the signal strength $\mu_{\wzjjew}$. The observed result is represented by the solid curve, while the dotted curve shows the result with only the statistical uncertainty included. The dashed curve represents the expected profile obtained from simulated data.\label{fig:NLL}}
\end{figure}


==> sections/auxiliaryDiagrams.tex <==

% 
% \begin{figure}[!htbp]
% \begin{center}
% \includegraphics[width=0.2\textwidth]{Diagrams/t_channel_LO_new.pdf} %\put(-50,200){{(a)}}
% \hspace*{0.3cm}\includegraphics[width=0.24\textwidth]{Diagrams/u_channel_LO_new.pdf} %\put(-50,200){{(b)}}
% \hspace*{0.3cm}\includegraphics[width=0.27\textwidth]{Diagrams/s_channel_LO_new.pdf} %\put(-50,200){{(b)}}
% \caption{Diagrams of \wz\ production in hadronic collisions by quark-antiquark annihilation at LO in QCD.
% }
% \label{fig:diag_LO}
% \end{center}
% \end{figure}


% 
% \begin{figure}[!htbp]
% \begin{center}
% \includegraphics[width=0.23\textwidth]{Diagrams/NLO_1_new.pdf} %\put(-50,200){{(a)}}
% \hspace*{0.3cm}\includegraphics[width=0.28\textwidth]{Diagrams/NLO_2_new.pdf} %\put(-50,200){{(b)}}
% \caption{Examples of two diagrams for NLO  QCD corrections to \wz\ production in hadronic collisions, from gluon bremsstrahlung in the final state.
% }
% \label{fig:diag_NLO}
% \end{center}
% \end{figure}
% 



\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.22\textwidth]{Diagrams/VBS_1_new.pdf} %\put(-50,200){{(a)}}
\hspace*{0.2cm}\includegraphics[width=0.22\textwidth]{Diagrams/VBS_4_new.pdf} %\put(-50,200){{(b)}}
\hspace*{0.2cm}\includegraphics[width=0.22\textwidth]{Diagrams/VBS_2_new.pdf} %\put(-50,200){{(b)}}
\hspace*{0.2cm}\hspace*{0.2cm}\includegraphics[width=0.22\textwidth]{Diagrams/VBS_3_new.pdf} %\put(-50,200){{(b)}}
\caption{Diagrams at \LO of the vector boson scattering process in hadronic collisions with a \wzjj final state.
}
\label{fig:diag_VBS}
\end{center}
\end{figure}



\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.25\textwidth]{Diagrams/tZ.pdf} %\put(-50,200){{(a)}}
\caption{Example diagram of $tZj$ production at \LO in QCD.
}
\label{fig:diag_tZ}
\end{center}
\end{figure}





==> sections/auxiliaryDiffXSections.tex <==
% \subsubsection{Additional differential cross section measurements, with \sherpa prediction scaled}
% 
% 
% \begin{figure}[!htbp]
% \begin{center}
% \includegraphics[width=0.45\textwidth]{Unfolding/mTWZ_xsection_notNorm_BinWidth__All.pdf}
% \caption{The measured \wzjj differential cross section in the VBS fiducial phase space as a function of \mtwz.
% %
% The inner and outer error bars on the data points represent the statistical and total uncertainties, respectively.
% The measurements are compared to the sum of the rescaled \wzjjqcd and \wzjjew predictions from \sherpa (red line).
% The \wzjjew and \wzjjqcd sub-contributions are also represented by dashed blue and dashed-dotted violet lines, respectively.
% %
% The right $y$-axis refers to the last cross section point, separated from the others by a vertical dashed line, as this last bin is integrated up to the maximum value reached in the phase space.
% %
% }
% \label{fig:diffXSection:mTWZ}
% \end{center}
% \end{figure}
% 
% 
% 
% 
% \begin{figure}[!htbp]
% \begin{center}
% \includegraphics[width=0.45\textwidth]{Unfolding/NjGap_xsection_notNorm_BinWidth__All.pdf}\put(-55,75){{(a)}}
% \includegraphics[width=0.45\textwidth]{Unfolding/dPhijj_xsection_notNorm_BinWidth__All.pdf}\put(-55,75){{(b)}}
% \caption{In (a), the measured \wzjj differential cross section in the VBS fiducial phase space as a function of as a function of \NjGap\, the exclusive jet multiplicity of jets with $p_\textrm{T} > 25$~\GeV in the gap between the two tagging jets.
% In (b), the measured \wzjj differential cross section in the VBS fiducial phase space as a function of \dPhijj\.
% The inner and outer error bars on the data points represent the statistical and total uncertainties, respectively.
% The measurements are compared to the sum of the rescaled \wzjjqcd and \wzjjew predictions from \sherpa (red line).
% The \wzjjew and \wzjjqcd sub-contributions are also represented by dashed blue and dashed-dotted violet lines, respectively.
% %
% The right $y$-axis refers to the last cross section point, separated from the others by a vertical dashed line, as this last bin is integrated up to the maximum value reached in the phase space.
% %
% }
% \label{fig:diffXSection:NjGap_dPhijj}
% \end{center}
% \end{figure}
% 
% 
% \clearpage
% \newpage



\subsubsection{Auxilliary figures with \sherpa prediction not scaled}




\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.45\textwidth]{Unfolding/SptL_xsection_notNorm_BinWidth_prefit__All.pdf}\put(-160,205){{(a)}}
\includegraphics[width=0.45\textwidth]{Unfolding/dPhiWZ_xsection_notNorm_BinWidth_prefit__All.pdf}\put(-160,205){{(b)}}
\caption{The measured \wzjj differential cross-section in the VBS fiducial phase space as a function of (a) \mtwz and (b) \dPhiWZ.
The inner and outer error bars on the data points represent the statistical and total uncertainties, respectively.
The measurements are compared with the sum of the \wzjjqcd and \wzjjew predictions from \sherpa (solid line).
The \wzjjew and \wzjjqcd sub-contributions are also represented by dashed and dashed-dotted lines, respectively.
%
In (a), the right $y$-axis refers to the last cross-section point, separated from the others by a vertical dashed line, as this last bin is integrated up to the maximum value reached in the phase space.
%
The lower panels show the ratios of the data to the predictions from \sherpa. 
}
\label{fig:diffXSection:SptL_dPhiWZ_prefit}
\end{center}
\end{figure}



\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.45\textwidth]{Unfolding/mTWZ_xsection_notNorm_BinWidth_prefit__All.pdf}
\caption{The measured \wzjj differential cross-section in the VBS fiducial phase space as a function of \mtwz.
%
The inner and outer error bars on the data points represent the statistical and total uncertainties, respectively.
The measurements are compared with the sum of the \wzjjqcd and \wzjjew predictions from \sherpa (solid line).
The \wzjjew and \wzjjqcd sub-contributions are also represented by dashed and dashed-dotted lines, respectively.
%
The right $y$-axis refers to the last cross-section point, separated from the others by a vertical dashed line, as this last bin is integrated up to the maximum value reached in the phase space.
%
The lower panel shows the ratio of the data to the prediction from \sherpa. 
}
\label{fig:diffXSection:mTWZ_prefit}
\end{center}
\end{figure}




\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.45\textwidth]{Unfolding/Njets40_xsection_notNorm_BinWidth_prefit__All.pdf}
\caption{The measured \wzjj differential cross-section in the VBS fiducial phase space as a function of the exclusive jet multiplicity of jets with $p_\textrm{T} > 40$~\GeV.
The inner and outer error bars on the data points represent the statistical and total uncertainties, respectively.
The measurements are compared with the sum of the \wzjjqcd and \wzjjew predictions from \sherpa (solid line).
The \wzjjew and \wzjjqcd sub-contributions are also represented by dashed and dashed-dotted lines, respectively.
%
The right $y$-axis refers to the last cross-section point, separated from the others by a vertical dashed line, as this last bin is integrated up to the maximum value reached in the phase space.
%
The lower panel shows the ratio of the data to the prediction from \sherpa. 
}
\label{fig:diffXSection:Njets_prefit}
\end{center}
\end{figure}




\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.45\textwidth]{Unfolding/dYjj40_xsection_notNorm_BinWidth_prefit__All.pdf}\put(-55,75){{(a)}}
\includegraphics[width=0.45\textwidth]{Unfolding/mjj40_xsection_notNorm_BinWidth_prefit__All.pdf}\put(-55,75){{(b)}}
\caption{The measured \wzjj differential cross-section in the VBS fiducial phase space as a function of (a) the absolute difference in rapidity between the two tagging jets \dYjj  and (b) the invariant mass of the tagging jets \mjj.
The inner and outer error bars on the data points represent the statistical and total uncertainties, respectively.
The measurements are compared with the sum of the \wzjjqcd and \wzjjew predictions from \sherpa (solid line).
The \wzjjew and \wzjjqcd sub-contributions are also represented by dashed and dashed-dotted lines, respectively.
%
In (b), the right $y$-axis refers to the last cross-section point, separated from the others by a vertical dashed line, as this last bin is integrated up to the maximum value reached in the phase space.
%
The lower panels show the ratios of the data to the predictions from \sherpa. 
}
\label{fig:diffXSection:dYjj_mjj_prefit}
\end{center}
\end{figure}




\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.45\textwidth]{Unfolding/NjGap_xsection_notNorm_BinWidth_prefit__All.pdf}\put(-55,75){{(a)}}
\includegraphics[width=0.45\textwidth]{Unfolding/dPhijj_xsection_notNorm_BinWidth_prefit__All.pdf}\put(-55,75){{(b)}}
\caption{The measured \wzjj differential cross-section in the VBS fiducial phase space as a function of (a) \NjGap\, the exclusive jet multiplicity of jets with $p_\textrm{T} > 25$~\GeV in the gap between the two tagging jets and (b) \dPhijj.
The inner and outer error bars on the data points represent the statistical and total uncertainties, respectively.
The measurements are compared with the sum of the \wzjjqcd and \wzjjew predictions from \sherpa (solid line).
The \wzjjew and \wzjjqcd sub-contributions are also represented by dashed and dashed-dotted lines, respectively.
%
The right $y$-axis refers to the last cross-section point, separated from the others by a vertical dashed line, as this last bin is integrated up to the maximum value reached in the phase space.
%
The lower panels show the ratios of the data to the predictions from \sherpa. 
}
\label{fig:diffXSection:NjGap_dPhijj_prefit}
\end{center}
\end{figure}



==> sections/auxiliaryInclXSections.tex <==
%%%%%% Cross section figures, Wp and Wm
\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=10cm]{AuxFigs/intXsectionFig_VBS.pdf}
\caption{Ratio between the measured \wzjj integrated cross-sections in the fiducial phase space and the SM prediction from \sherpa in each of the four channels and for their combination. 
%
The inner and outer error bars on the data points represent the statistical and total uncertainties, respectively.
%
The hatched band represents the uncertainty associated to the \sherpa prediction, which is dominated by the QCD scale uncertainty.
}
\label{fig:int_wzjj_cross_section}
\end{center}
\end{figure}



==> sections/diffXsectionTables.tex <==

\begin{table}[!htbp]
\caption{Measured \wzjj  differential cross-section in the VBS fiducial phase space as a function of \mtwz.
The relative uncertainties are reported as percentages.
The decomposition of the total systematic uncertainty into the main sources correlated between channels and the source uncorrelated between channels is indicated in the bottom rows.
\label{tab:DiffXSection:mTWZ}}
\begin{center}
%\resizebox{1.\textwidth}{!}{
\input{tables/Diff_XSections_VBS/mTWZ_xsection_notNorm_BinWidth__All.tex}
%}
\end{center}
\end{table}



\begin{table}[!htbp]
\caption{Correlation matrix of the unfolded fiducial cross-section as a function of  \mtwz.
\label{tab:CovMatrix:mTWZ}}
\begin{center}
%\resizebox{1.\textwidth}{!}{
\input{tables/Diff_XSections_VBS/mTWZ_xsection_notNorm_BinWidth__All_covMatrix.tex}
%}
\end{center}
\end{table}




\begin{table}[!htbp]
\caption{Measured \wzjj  differential cross-section in the VBS fiducial phase space as a function of \sptl.
The relative uncertainties are reported as percentages.
The decomposition of the total systematic uncertainty into the main sources correlated between channels and the source uncorrelated between channels is indicated in the bottom rows.
\label{tab:DiffXSection:SptL}}
\begin{center}
%\resizebox{1.\textwidth}{!}{
\input{tables/Diff_XSections_VBS/SptL_xsection_notNorm_BinWidth__All.tex}
%}
\end{center}
\end{table}


\begin{table}[!htbp]
\caption{Correlation matrix of the unfolded fiducial cross-section as a function of  \sptl.
\label{tab:CovMatrix:SptL}}
\begin{center}
%\resizebox{1.\textwidth}{!}{
\input{tables/Diff_XSections_VBS/SptL_xsection_notNorm_BinWidth__All_covMatrix.tex}
%}
\end{center}
\end{table}




\begin{table}[!htbp]
\caption{Measured \wzjj differential cross-section in the fiducial phase space as a function of \dPhiWZ.
The relative uncertainties are reported as percentages.
The decomposition of the total systematic uncertainty into the main sources correlated between channels and the source uncorrelated between channels is indicated in the bottom rows.
\label{tab:DiffXSection:dPhiWZ}}
\begin{center}
%\resizebox{1.\textwidth}{!}{
\input{tables/Diff_XSections_VBS/dPhiWZ_xsection_notNorm_BinWidth__All.tex}
%}
\end{center}
\end{table}



\begin{table}[!htbp]
\caption{Correlation matrix of the unfolded fiducial cross-section as a function of \dPhiWZ.   
\label{tab:CovMatrix:dPhiWZ}}
\begin{center}
%\resizebox{1.\textwidth}{!}{
\input{tables/Diff_XSections_VBS/dPhiWZ_xsection_notNorm_BinWidth__All_covMatrix.tex}
%}
\end{center}
\end{table}



\begin{table}[!htbp]
\caption{Measured $W^{\pm}Z$jj  differential cross-section in the fiducial phase space as a function of \njets for jets with a $p_{\mathrm{T}} > 40$~\GeV.
The relative uncertainties are reported as percentages.
The decomposition of the total systematic uncertainty into the main sources correlated between channels and the source uncorrelated between channels is indicated in the bottom rows.
\label{tab:DiffXSection:Njets40}}
\begin{center}
%\resizebox{1.\textwidth}{!}{
\input{tables/Diff_XSections_VBS/Njets40_xsection_notNorm_BinWidth__All.tex}
%}
\end{center}
\end{table}



\begin{table}[!htbp]
\caption{Correlation matrix of the unfolded fiducial cross-section as a function of \njets for jets with a $p_{\mathrm{T}} > 40$~\GeV.
\label{tab:CovMatrix:Njets40}}
\begin{center}
%\resizebox{1.\textwidth}{!}{
\input{tables/Diff_XSections_VBS/Njets40_xsection_notNorm_BinWidth__All_covMatrix.tex}
%}
\end{center}
\end{table}




\begin{table}[!htbp]
\caption{Measured \wzjj  differential cross-section in the VBS fiducial phase space as a function of \mjj for jets with a $p_{\mathrm{T}} > 40$~\GeV.
The relative uncertainties are reported as percentages.
The decomposition of the total systematic uncertainty into the main sources correlated between channels and the source uncorrelated between channels is indicated in the bottom rows.
\label{tab:DiffXSection:Mjj40}}
\begin{center}
%\resizebox{1.\textwidth}{!}{
\input{tables/Diff_XSections_VBS/mjj40_xsection_notNorm_BinWidth__All.tex}
%}
\end{center}
\end{table}




\begin{table}[!htbp]
\caption{Correlation matrix of the unfolded fiducial cross-section as a function of \mjj for jets with a $p_{\mathrm{T}} > 40$~\GeV.
\label{tab:CovMatrix:mjj40}}
\begin{center}
%\resizebox{1.\textwidth}{!}{
\input{tables/Diff_XSections_VBS/mjj40_xsection_notNorm_BinWidth__All_covMatrix.tex}
%}
\end{center}
\end{table}



\begin{table}[!htbp]
\caption{Measured \wzjj  differential cross-section in the VBS fiducial phase space as a function of \dYjj\ for jets with a $p_{\mathrm{T}} > 40$~\GeV.
The relative uncertainties are reported as percentages.
The decomposition of the total systematic uncertainty into the main sources correlated between channels and the source uncorrelated between channels is indicated in the bottom rows.
\label{tab:DiffXSection:dYjj40}}
\begin{center}
%\resizebox{1.\textwidth}{!}{
\input{tables/Diff_XSections_VBS/dYjj40_xsection_notNorm_BinWidth__All.tex}
%}
\end{center}
\end{table}



\begin{table}[!htbp]
\caption{Correlation matrix of the unfolded fiducial cross-section as a function of \dYjj\ for jets with a $p_{\mathrm{T}} > 40$~\GeV.
\label{tab:CovMatrix:dYjj40}}
\begin{center}
%\resizebox{1.\textwidth}{!}{
\input{tables/Diff_XSections_VBS/dYjj40_xsection_notNorm_BinWidth__All_covMatrix.tex}
%}
\end{center}
\end{table}



\begin{table}[!htbp]
\caption{Measured \wzjj  differential cross-section in the VBS fiducial phase space as a function of \dPhijj\ for jets with a $p_{\mathrm{T}} > 40$~\GeV.
The relative uncertainties are reported as percentages.
The decomposition of the total systematic uncertainty into the main sources correlated between channels and the source uncorrelated between channels is indicated in the bottom rows.
\label{tab:DiffXSection:dPhijj}}
\begin{center}
%\resizebox{1.\textwidth}{!}{
\input{tables/Diff_XSections_VBS/dPhijj_xsection_notNorm_BinWidth__All.tex}
%}
\end{center}
\end{table}



\begin{table}[!htbp]
\caption{Correlation matrix of the unfolded fiducial cross-section as a function of \dPhijj\ for jets with a $p_{\mathrm{T}} > 40$~\GeV.
\label{tab:CovMatrix:dPhijj}}
\begin{center}
%\resizebox{1.\textwidth}{!}{
\input{tables/Diff_XSections_VBS/dPhijj_xsection_notNorm_BinWidth__All_covMatrix.tex}
%}
\end{center}
\end{table}



\begin{table}[!htbp]
\caption{Measured \wzjj  differential cross-section in the VBS fiducial phase space as a function of \NjGap\, the exclusive jet multiplicity of jets with $p_\textrm{T} > 25$~\GeV in the gap between the two tagging jets.
The relative uncertainties are reported as percentages.
The decomposition of the total systematic uncertainty into the main sources correlated between channels and the source uncorrelated between channels is indicated in the bottom rows.
\label{tab:DiffXSection:NjGap}}
\begin{center}
%\resizebox{1.\textwidth}{!}{
\input{tables/Diff_XSections_VBS/NjGap_xsection_notNorm_BinWidth__All.tex}
%}
\end{center}
\end{table}



\begin{table}[!htbp]
\caption{Correlation matrix of the unfolded fiducial cross-section as a function of \NjGap\, the exclusive jet multiplicity of jets with $p_\textrm{T} > 25$~\GeV in the gap between the two tagging jets.
\label{tab:CovMatrix:NjGap}}
\begin{center}
%\resizebox{1.\textwidth}{!}{
\input{tables/Diff_XSections_VBS/NjGap_xsection_notNorm_BinWidth__All_covMatrix.tex}
%}
\end{center}
\end{table}


==> sections/postFitControlDist.tex <==
\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.38\textwidth]{AuxFigs/hWZVBS_SR_aZylW_lin_ratio_overF_1516.pdf}\put(-30,110){{(a)}}
\includegraphics[width=0.38\textwidth]{AuxFigs/hWZVBS_SR_centrality_lin_ratio_overF_1516.pdf}\put(-30,110){{(b)}}\\
\includegraphics[width=0.38\textwidth]{AuxFigs/hWZVBS_SR_RpThard2_lin_ratio_overF_1516.pdf}\put(-30,110){{(c)}}
\includegraphics[width=0.38\textwidth]{AuxFigs/hWZVBS_SR_Njets_lin_ratio_overF_1516.pdf}\put(-30,110){{(d)}}\\
\includegraphics[width=0.38\textwidth]{AuxFigs/hWZVBS_SR_Dphi_jj_lin_ratio_1516.pdf}\put(-75,145){{(e)}}
\caption{Post-fit distributions in the signal region of the five most important variable of the BDT discriminant, by decreasing order of importance in the BDT ranking (a) $|y_Z - y_{\ell,W}|$, (b) $\zeta_{\mathrm{lep.}}$, (c) $R_{p_\mathrm{T}}^{\mathrm{hard}}$, (d) the multiplicity of jets with $p_\mathrm{T} > 25$~\GeV\ and (e) $\Delta \phi_{jj}$. 
%
Signal and backgrounds are normalised to the expected number of events after the fit. 
%
The uncertainty band around the MC expectation includes all systematic uncertainties as obtained from the fit.
%
}
\label{fig:postFitControlDists}
\end{center}
\end{figure}





\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.38\textwidth]{AuxFigs/hWZVBS_CRQCD_aZylW_lin_ratio_overF_1516.pdf}\put(-30,110){{(a)}}
\includegraphics[width=0.38\textwidth]{AuxFigs/hWZVBS_CRQCD_centrality_lin_ratio_overF_1516.pdf}\put(-30,110){{(b)}}\\
\includegraphics[width=0.38\textwidth]{AuxFigs/hWZVBS_CRQCD_RpThard2_lin_ratio_overF_1516.pdf}\put(-30,110){{(c)}}
\includegraphics[width=0.38\textwidth]{AuxFigs/hWZVBS_CRQCD_Njets_lin_ratio_overF_1516.pdf}\put(-30,110){{(d)}}\\
\includegraphics[width=0.38\textwidth]{AuxFigs/hWZVBS_CRQCD_Dphi_jj_lin_ratio_1516.pdf}\put(-75,145){{(e)}}
\caption{Post-fit distributions in the \wzjj-QCD CR region of the five most important variable of the BDT discriminant, by decreasing order of importance in the BDT ranking (a) $|y_Z - y_{\ell,W}|$, (b) $\zeta_{\mathrm{lep.}}$, (c) $R_{p_\mathrm{T}}^{\mathrm{hard}}$, (d) the multiplicity of jets with $p_\mathrm{T} > 25$~\GeV\ and (e) $\Delta \phi_{jj}$. 
%
Signal and backgrounds are normalised to the expected number of events after the fit. 
%
The uncertainty band around the MC expectation includes all systematic uncertainties as obtained from the fit.
%
}
\label{fig:postFitControlDists_QCDCR}
\end{center}
\end{figure}



\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.38\textwidth]{AuxFigs/hWZVBS_CRQCD_mJJ_fit_lin_ratio_overF_1516.pdf}
\caption{Post-fit distributions in the \wzjj-QCD CR region of the invariant of the two tagging jets $m_{jj}$. 
%
Signal and backgrounds are normalised to the expected number of events after the fit. 
%
The uncertainty band around the MC expectation includes all systematic uncertainties as obtained from the fit.
%
}
\label{fig:postFitControlDists_QCDCR_mjj}
\end{center}
\end{figure}





==> tables/Diff_XSections_VBS/NjGap_xsection_notNorm_BinWidth__All.tex <==
\begin{tabular}{l r r r r} 
\toprule 
$N_{\mathrm{jets}}^{\mathrm{gap}}$ & $0$ -- $0$ &$0$ -- $1$ &$1$ -- $2$ &$\geq 2$ \\\midrule 
 $\Delta \sigma_{W^{\pm}Zjj}^{\mathrm{fid.}}$ [fb]& $0.88$ & $0.55$ & $0.11$ & $0.13$ \\ 
\midrule 
\multicolumn{5}{c}{Relative Uncertainties [\%]}\\ 
\midrule 
 Statistics& $14.9$ & $20.4$ & $48.5$ & $44.5$ \\ 
 All systematics& $8.5$ & $12.9$ & $33.8$ & $18.3$ \\ 
 Luminosity& $2.5$ & $2.5$ & $3.2$ & $2.6$ \\ 
\midrule 
 Total& $17.1$ & $24.2$ & $59.1$ & $48.2$ \\ 
\midrule 
\midrule 
 Uncorrelated syst.& $1.0$ & $1.2$ & $4.5$ & $3.1$ \\ 
\midrule 
 Unfolding& $0.2$ & $2.5$ & $21.6$ & $7.1$ \\ 
 Electrons& $1.5$ & $1.4$ & $1.5$ & $1.4$ \\ 
 Muons& $1.8$ & $1.8$ & $1.9$ & $2.0$ \\ 
 Jets& $4.3$ & $9.1$ & $14.4$ & $12.6$ \\ 
 Red. Background& $2.0$ & $3.4$ & $12.2$ & $4.9$ \\ 
 Irred. Background& $5.9$ & $6.9$ & $16.1$ & $8.2$ \\ 
 Pileup& $0.9$ & $0.3$ & $1.3$ & $0.7$ \\ 
\bottomrule 
\end{tabular} 


==> tables/Diff_XSections_VBS/NjGap_xsection_notNorm_BinWidth__All_covMatrix.tex <==
\begin{tabular}{l | r r r r} 
\toprule 
$N_{\mathrm{jets}}^{\mathrm{gap}}$ & $0$ -- $0$ &$0$ -- $1$ &$1$ -- $2$ &$\geq 2$ \\\midrule 
$0$ -- $0$ & $1.00$ & $0.09$ & $0.12$ & $0.10$ \\ 
$0$ -- $1$ & $0.09$ & $1.00$ & $0.26$ & $0.07$ \\ 
$1$ -- $2$ & $0.12$ & $0.26$ & $1.00$ & $0.23$ \\ 
$\geq 2$ & $0.10$ & $0.07$ & $0.23$ & $1.00$ \\ 
\bottomrule 
\end{tabular} 


==> tables/Diff_XSections_VBS/Njets40_xsection_notNorm_BinWidth__All.tex <==
\begin{tabular}{l r r r r} 
\toprule 
$N_{{\mathrm{jets}}}$  & $1$ -- $2$ &$2$ -- $3$ &$3$ -- $4$ &$\geq 4$ \\\midrule 
 $\Delta \sigma_{W^{\pm}Zjj}^{\mathrm{fid.}}$ [fb]& $0.92$ & $0.52$ & $0.09$ & $0.12$ \\ 
\midrule 
\multicolumn{5}{c}{Relative Uncertainties [\%]}\\ 
\midrule 
 Statistics& $14.2$ & $21.6$ & $64.7$ & $49.3$ \\ 
 All systematics& $8.0$ & $13.3$ & $31.7$ & $19.2$ \\ 
 Luminosity& $2.5$ & $2.6$ & $3.4$ & $2.8$ \\ 
\midrule 
 Total& $16.3$ & $25.3$ & $72.0$ & $52.9$ \\ 
\midrule 
\midrule 
 Uncorrelated syst.& $1.0$ & $1.4$ & $4.9$ & $4.2$ \\ 
\midrule 
 Unfolding& $0.1$ & $1.1$ & $15.7$ & $3.0$ \\ 
 Electrons& $1.4$ & $1.5$ & $1.5$ & $1.6$ \\ 
 Muons& $1.8$ & $1.8$ & $2.1$ & $1.9$ \\ 
 Jets& $3.8$ & $9.2$ & $15.3$ & $12.7$ \\ 
 Red. Background& $2.1$ & $3.8$ & $8.9$ & $7.2$ \\ 
 Irred. Background& $5.5$ & $7.5$ & $19.4$ & $9.9$ \\ 
 Pileup& $1.2$ & $0.2$ & $2.1$ & $1.8$ \\ 
\bottomrule 
\end{tabular} 


==> tables/Diff_XSections_VBS/Njets40_xsection_notNorm_BinWidth__All_covMatrix.tex <==
\begin{tabular}{l | r r r r} 
\toprule 
$N_{{\mathrm{jets}}}$  & $1$ -- $2$ &$2$ -- $3$ &$3$ -- $4$ &$\geq 4$ \\\midrule 
$1$ -- $2$ & $1.00$ & $0.09$ & $0.15$ & $0.16$ \\ 
$2$ -- $3$ & $0.09$ & $1.00$ & $0.12$ & $0.11$ \\ 
$3$ -- $4$ & $0.15$ & $0.12$ & $1.00$ & $0.04$ \\ 
$\geq 4$ & $0.16$ & $0.11$ & $0.04$ & $1.00$ \\ 
\bottomrule 
\end{tabular} 


==> tables/Diff_XSections_VBS/SptL_xsection_notNorm_BinWidth__All.tex <==
\begin{tabular}{l r r r r r} 
\toprule 
$\sum p_\mathrm{T}^{\ell}$ [GeV] & $60$ -- $150$ &$150$ -- $250$ &$250$ -- $350$ &$350$ -- $500$ &$\geq 500$ \\\midrule 
 $\Delta \sigma_{W^{\pm}Zjj}^{\mathrm{fid.}}$ [fb]& $0.14$ & $0.91$ & $0.38$ & $0.16$ & $0.09$ \\ 
\midrule 
\multicolumn{6}{c}{Relative Uncertainties [\%]}\\ 
\midrule 
 Statistics& $22.6$ & $13.8$ & $16.6$ & $23.5$ & $43.0$ \\ 
 All systematics& $23.8$ & $26.4$ & $11.6$ & $26.2$ & $33.6$ \\ 
 Luminosity& $2.9$ & $2.7$ & $2.4$ & $2.3$ & $2.2$ \\ 
\midrule 
 Total& $32.8$ & $29.8$ & $20.3$ & $35.2$ & $54.5$ \\ 
\midrule 
\midrule 
 Uncorrelated syst.& $1.8$ & $1.1$ & $0.7$ & $0.9$ & $1.7$ \\ 
\midrule 
 Unfolding& $14.8$ & $23.2$ & $9.1$ & $25.1$ & $32.4$ \\ 
 Electrons& $1.6$ & $1.2$ & $1.8$ & $2.6$ & $3.7$ \\ 
 Muons& $1.6$ & $1.5$ & $2.1$ & $2.9$ & $3.7$ \\ 
 Jets& $9.7$ & $6.9$ & $4.6$ & $3.1$ & $2.7$ \\ 
 Red. Background& $7.7$ & $4.5$ & $0.5$ & $0.1$ & $2.3$ \\ 
 Irred. Background& $12.6$ & $8.6$ & $3.8$ & $3.2$ & $2.3$ \\ 
 Pileup& $1.6$ & $1.2$ & $1.2$ & $3.2$ & $3.4$ \\ 
\bottomrule 
\end{tabular} 


==> tables/Diff_XSections_VBS/SptL_xsection_notNorm_BinWidth__All_covMatrix.tex <==
\begin{tabular}{l | r r r r r} 
\toprule 
$\sum p_\mathrm{T}^{\ell}$ [GeV] & $60$ -- $150$ &$150$ -- $250$ &$250$ -- $350$ &$350$ -- $500$ &$\geq 500$ \\\midrule 
$60$ -- $150$ & $1.00$ & $0.79$ & $0.06$ & $0.00$ & $0.01$ \\ 
$150$ -- $250$ & $0.79$ & $1.00$ & $0.30$ & $-0.02$ & $-0.07$ \\ 
$250$ -- $350$ & $0.06$ & $0.30$ & $1.00$ & $0.62$ & $0.06$ \\ 
$350$ -- $500$ & $0.00$ & $-0.02$ & $0.62$ & $1.00$ & $0.44$ \\ 
$\geq 500$ & $0.01$ & $-0.07$ & $0.06$ & $0.44$ & $1.00$ \\ 
\bottomrule 
\end{tabular} 


==> tables/Diff_XSections_VBS/dPhiWZ_xsection_notNorm_BinWidth__All.tex <==
\begin{tabular}{l r r r r r} 
\toprule 
$\Delta\phi(W,Z)$ [rad] & $0.0$ -- $0.6$ &$0.6$ -- $1.2$ &$1.2$ -- $1.8$ &$1.8$ -- $2.5$ &$2.5$ - $3.15$ \\\midrule 
 $\Delta \sigma_{W^{\pm}Zjj}^{\mathrm{fid.}}$ [fb]& $0.30$ & $0.37$ & $0.28$ & $0.40$ & $0.32$ \\ 
\midrule 
\multicolumn{6}{c}{Relative Uncertainties [\%]}\\ 
\midrule 
 Statistics& $26.6$ & $23.8$ & $28.3$ & $23.7$ & $27.9$ \\ 
 All systematics& $11.7$ & $9.5$ & $10.9$ & $10.0$ & $13.9$ \\ 
 Luminosity& $2.5$ & $2.4$ & $2.6$ & $2.6$ & $2.8$ \\ 
\midrule 
 Total& $29.1$ & $25.6$ & $30.3$ & $25.7$ & $31.2$ \\ 
\midrule 
\midrule 
 Uncorrelated syst.& $1.9$ & $1.2$ & $1.5$ & $1.3$ & $2.0$ \\ 
\midrule 
 Unfolding& $0.2$ & $0.2$ & $0.1$ & $0.1$ & $0.1$ \\ 
 Electrons& $1.6$ & $1.4$ & $1.5$ & $1.5$ & $1.6$ \\ 
 Muons& $2.1$ & $2.0$ & $1.9$ & $1.8$ & $1.9$ \\ 
 Jets& $7.4$ & $6.5$ & $6.0$ & $5.2$ & $7.1$ \\ 
 Red. Background& $4.3$ & $2.9$ & $2.7$ & $2.2$ & $4.5$ \\ 
 Irred. Background& $6.1$ & $4.7$ & $7.3$ & $7.0$ & $9.9$ \\ 
 Pileup& $2.0$ & $0.9$ & $0.9$ & $0.5$ & $0.5$ \\ 
\bottomrule 
\end{tabular} 


==> tables/Diff_XSections_VBS/dPhiWZ_xsection_notNorm_BinWidth__All_covMatrix.tex <==
\begin{tabular}{l | r r r r r} 
\toprule 
$\Delta\phi(W,Z)$ [rad] & $0.0$ -- $0.6$ &$0.6$ -- $1.2$ &$1.2$ -- $1.8$ &$1.8$ -- $2.5$ &$2.5$ - $3.15$ \\\midrule 
$0.0$ -- $0.6$ & $1.00$ & $0.04$ & $0.06$ & $0.12$ & $0.13$ \\ 
$0.6$ -- $1.2$ & $0.04$ & $1.00$ & $0.17$ & $0.02$ & $0.12$ \\ 
$1.2$ -- $1.8$ & $0.06$ & $0.17$ & $1.00$ & $0.14$ & $0.07$ \\ 
$1.8$ -- $2.5$ & $0.12$ & $0.02$ & $0.14$ & $1.00$ & $0.07$ \\ 
$2.5$ -- $3.1$ & $0.13$ & $0.12$ & $0.07$ & $0.07$ & $1.00$ \\ 
\bottomrule 
\end{tabular} 


==> tables/Diff_XSections_VBS/dPhijj_xsection_notNorm_BinWidth__All.tex <==
\begin{tabular}{l r r r r r} 
\toprule 
$\Delta\phi_{jj}$ [rad] & $0.0$ -- $1.0$ &$1.0$ -- $1.8$ &$1.8$ -- $2.3$ &$2.3$ -- $2.8$ &$2.8$ - $3.15$ \\\midrule 
 $\Delta \sigma_{W^{\pm}Zjj}^{\mathrm{fid.}}$ [fb]& $0.28$ & $0.24$ & $0.28$ & $0.53$ & $0.35$ \\ 
\midrule 
\multicolumn{6}{c}{Relative Uncertainties [\%]}\\ 
\midrule 
 Statistics& $24.6$ & $28.1$ & $27.7$ & $18.5$ & $24.3$ \\ 
 All systematics& $12.5$ & $12.1$ & $11.5$ & $9.1$ & $11.4$ \\ 
 Luminosity& $2.5$ & $2.6$ & $2.6$ & $2.5$ & $2.7$ \\ 
\midrule 
 Total& $27.6$ & $30.6$ & $30.0$ & $20.7$ & $26.8$ \\ 
\midrule 
\midrule 
 Uncorrelated syst.& $2.3$ & $2.9$ & $2.4$ & $1.2$ & $1.9$ \\ 
\midrule 
 Unfolding& $0.1$ & $0.1$ & $0.0$ & $0.0$ & $0.7$ \\ 
 Electrons& $1.6$ & $1.6$ & $1.5$ & $1.4$ & $1.3$ \\ 
 Muons& $1.9$ & $1.9$ & $1.8$ & $1.7$ & $1.8$ \\ 
 Jets& $9.1$ & $7.2$ & $6.3$ & $5.3$ & $4.4$ \\ 
 Red. Background& $3.4$ & $4.2$ & $4.3$ & $2.4$ & $2.9$ \\ 
 Irred. Background& $6.1$ & $7.2$ & $7.2$ & $5.7$ & $9.1$ \\ 
 Pileup& $0.5$ & $0.7$ & $1.4$ & $1.1$ & $0.8$ \\ 
\bottomrule 
\end{tabular} 


==> tables/Diff_XSections_VBS/dPhijj_xsection_notNorm_BinWidth__All_covMatrix.tex <==
\begin{tabular}{l | r r r r r} 
\toprule 
$\Delta\phi_{jj}$ [rad] & $0.0$ -- $1.0$ &$1.0$ -- $1.8$ &$1.8$ -- $2.3$ &$2.3$ -- $2.8$ &$2.8$ - $3.15$ \\\midrule 
$0.0$ -- $1.0$ & $1.00$ & $0.13$ & $0.15$ & $0.17$ & $0.16$ \\ 
$1.0$ -- $1.8$ & $0.13$ & $1.00$ & $0.09$ & $0.13$ & $0.16$ \\ 
$1.8$ -- $2.3$ & $0.15$ & $0.09$ & $1.00$ & $0.10$ & $0.15$ \\ 
$2.3$ -- $2.8$ & $0.17$ & $0.13$ & $0.10$ & $1.00$ & $0.17$ \\ 
$2.8$ -- $3.1$ & $0.16$ & $0.16$ & $0.15$ & $0.17$ & $1.00$ \\ 
\bottomrule 
\end{tabular} 


==> tables/Diff_XSections_VBS/dYjj40_xsection_notNorm_BinWidth__All.tex <==
\begin{tabular}{l r r r r} 
\toprule 
$\Delta y_{jj}$ [rad] & $0.0$ -- $2.5$ &$2.5$ -- $3.5$ &$3.5$ -- $4.5$ &$4.5$ - $7.0$ \\\midrule 
 $\Delta \sigma_{W^{\pm}Zjj}^{\mathrm{fid.}}$ [fb]& $0.40$ & $0.36$ & $0.61$ & $0.32$ \\ 
\midrule 
\multicolumn{5}{c}{Relative Uncertainties [\%]}\\ 
\midrule 
 Statistics& $21.9$ & $23.1$ & $17.1$ & $24.0$ \\ 
 All systematics& $7.8$ & $11.0$ & $9.6$ & $16.1$ \\ 
 Luminosity& $2.4$ & $2.7$ & $2.5$ & $2.7$ \\ 
\midrule 
 Total& $23.2$ & $25.6$ & $19.6$ & $28.9$ \\ 
\midrule 
\midrule 
 Uncorrelated syst.& $1.8$ & $2.2$ & $1.2$ & $2.5$ \\ 
\midrule 
 Unfolding& $0.0$ & $1.5$ & $0.0$ & $0.0$ \\ 
 Electrons& $1.6$ & $1.5$ & $1.4$ & $1.4$ \\ 
 Muons& $1.9$ & $1.8$ & $1.8$ & $1.8$ \\ 
 Jets& $3.3$ & $4.5$ & $6.2$ & $10.7$ \\ 
 Red. Background& $3.2$ & $4.0$ & $2.2$ & $4.3$ \\ 
 Irred. Background& $4.6$ & $7.9$ & $5.8$ & $9.9$ \\ 
 Pileup& $1.3$ & $1.1$ & $0.3$ & $1.5$ \\ 
\bottomrule 
\end{tabular} 


==> tables/Diff_XSections_VBS/dYjj40_xsection_notNorm_BinWidth__All_covMatrix.tex <==
\begin{tabular}{l | r r r r} 
\toprule 
$\Delta y_{jj}$ [rad] & $0.0$ -- $2.5$ &$2.5$ -- $3.5$ &$3.5$ -- $4.5$ &$4.5$ - $7.0$ \\\midrule 
$0.0$ -- $2.5$ & $1.00$ & $0.10$ & $0.12$ & $0.13$ \\ 
$2.5$ -- $3.5$ & $0.10$ & $1.00$ & $0.15$ & $0.22$ \\ 
$3.5$ -- $4.5$ & $0.12$ & $0.15$ & $1.00$ & $0.20$ \\ 
$4.5$ -- $7.0$ & $0.13$ & $0.22$ & $0.20$ & $1.00$ \\ 
\bottomrule 
\end{tabular} 


==> tables/Diff_XSections_VBS/mTWZ_xsection_notNorm_BinWidth__All.tex <==
\begin{tabular}{l r r r r r} 
\toprule 
$m_{\mathrm{T}}^{WZ}$ [GeV] & $150$ -- $200$ &$200$ -- $250$ &$250$ -- $300$ &$300$ -- $400$ &$\geq 400$ \\\midrule 
 $\Delta \sigma_{W^{\pm}Zjj}^{\mathrm{fid.}}$ [fb]& $0.49$ & $0.64$ & $0.24$ & $0.21$ & $0.06$ \\ 
\midrule 
\multicolumn{6}{c}{Relative Uncertainties [\%]}\\ 
\midrule 
 Statistics& $24.7$ & $19.3$ & $31.0$ & $33.6$ & $63.1$ \\ 
 All systematics& $16.9$ & $11.8$ & $10.6$ & $9.9$ & $18.4$ \\ 
 Luminosity& $2.8$ & $2.3$ & $2.4$ & $2.5$ & $3.0$ \\ 
\midrule 
 Total& $29.9$ & $22.6$ & $32.7$ & $35.0$ & $65.7$ \\ 
\midrule 
\midrule 
 Uncorrelated syst.& $4.2$ & $0.7$ & $1.0$ & $1.4$ & $5.6$ \\ 
\midrule 
 Unfolding& $5.2$ & $9.1$ & $6.0$ & $2.0$ & $8.6$ \\ 
 Electrons& $1.5$ & $1.4$ & $2.0$ & $2.3$ & $3.0$ \\ 
 Muons& $1.8$ & $1.9$ & $2.2$ & $2.3$ & $3.5$ \\ 
 Jets& $8.0$ & $5.5$ & $6.0$ & $6.5$ & $3.4$ \\ 
 Red. Background& $6.1$ & $0.5$ & $0.5$ & $1.9$ & $5.5$ \\ 
 Irred. Background& $10.6$ & $3.0$ & $4.3$ & $4.6$ & $11.9$ \\ 
 Pileup& $1.4$ & $0.8$ & $0.9$ & $0.8$ & $1.4$ \\ 
\bottomrule 
\end{tabular} 


==> tables/Diff_XSections_VBS/mTWZ_xsection_notNorm_BinWidth__All_covMatrix.tex <==
\begin{tabular}{l | r r r r r} 
\toprule 
$m_{\mathrm{T}}^{WZ}$ [GeV] & $150$ -- $200$ &$200$ -- $250$ &$250$ -- $300$ &$300$ -- $400$ &$\geq 400$ \\\midrule 
$150$ -- $200$ & $1.00$ & $-0.02$ & $0.02$ & $0.14$ & $0.07$ \\ 
$200$ -- $250$ & $-0.02$ & $1.00$ & $0.05$ & $-0.06$ & $0.04$ \\ 
$250$ -- $300$ & $0.02$ & $0.05$ & $1.00$ & $0.00$ & $0.02$ \\ 
$300$ -- $400$ & $0.14$ & $-0.06$ & $0.00$ & $1.00$ & $-0.06$ \\ 
$\geq 400$ & $0.07$ & $0.04$ & $0.02$ & $-0.06$ & $1.00$ \\ 
\bottomrule 
\end{tabular} 


==> tables/Diff_XSections_VBS/mjj40_xsection_notNorm_BinWidth__All.tex <==
\begin{tabular}{l r r r r} 
\toprule 
$m_{jj}$ [GeV] & $500$ -- $700$ &$700$ -- $1000$ &$1000$ -- $1500$ &$\geq 1500$ \\\midrule 
 $\Delta \sigma_{W^{\pm}Zjj}^{\mathrm{fid.}}$ [fb]& $0.55$ & $0.51$ & $0.48$ & $0.16$ \\ 
\midrule 
\multicolumn{5}{c}{Relative Uncertainties [\%]}\\ 
\midrule 
 Statistics& $19.7$ & $21.6$ & $20.5$ & $36.9$ \\ 
 All systematics& $11.7$ & $10.1$ & $11.4$ & $16.8$ \\ 
 Luminosity& $2.7$ & $2.6$ & $2.4$ & $2.7$ \\ 
\midrule 
 Total& $22.9$ & $23.9$ & $23.4$ & $40.5$ \\ 
\midrule 
\midrule 
 Uncorrelated syst.& $1.6$ & $1.4$ & $1.4$ & $2.6$ \\ 
\midrule 
 Unfolding& $0.0$ & $0.1$ & $0.2$ & $3.5$ \\ 
 Electrons& $1.4$ & $1.4$ & $1.5$ & $2.0$ \\ 
 Muons& $1.7$ & $1.7$ & $2.0$ & $1.8$ \\ 
 Jets& $5.4$ & $5.1$ & $9.1$ & $12.4$ \\ 
 Red. Background& $4.3$ & $3.4$ & $2.6$ & $1.1$ \\ 
 Irred. Background& $8.5$ & $6.9$ & $4.3$ & $9.1$ \\ 
 Pileup& $0.1$ & $0.7$ & $1.9$ & $1.3$ \\ 
\bottomrule 
\end{tabular} 


==> tables/Diff_XSections_VBS/mjj40_xsection_notNorm_BinWidth__All_covMatrix.tex <==
\begin{tabular}{l | r r r r} 
\toprule 
$m_{jj}$ [GeV] & $500$ -- $700$ &$700$ -- $1000$ &$1000$ -- $1500$ &$\geq 1500$ \\\midrule 
$500$ -- $700$ & $1.00$ & $0.11$ & $0.20$ & $0.18$ \\ 
$700$ -- $1000$ & $0.11$ & $1.00$ & $0.07$ & $0.13$ \\ 
$1000$ -- $1500$ & $0.20$ & $0.07$ & $1.00$ & $0.12$ \\ 
$\geq 1500$ & $0.18$ & $0.13$ & $0.12$ & $1.00$ \\ 
\bottomrule 
\end{tabular} 

